Approximated Structured Prediction for Learning Large Scale Graphical Models

This manuscripts contains the proofs for "A Primal-Dual Message-Passing Algorithm for Approximated Large Scale Structured Prediction".

==> sup_structured.tex <==
%\section{Regularized Structured Loss Minimization}
%\label{sec:reg}

%Consider a supervised learning setting with objects $x \in X$ and labels $y \in \Y$. In structured prediction  the labels may be sequences, trees, grids, or other high-dimensional objects with internal structure. Consider a function $\Phi: \X \times \Y \rightarrow \R^d$ that maps $(x,y)$ pairs to feature vectors. Our goal is to construct a linear prediction rule $$y_{\bftheta}(x) = \argmax{y \in \Y} \bftheta^\top \Phi(x,y)$$ with parameters $\bftheta \in \R^d$, such that $y_{\bftheta}(x)$ is a good approximation to the true label of $x$. The parameters $\bftheta$ are typically learned by minimizing the regularized loss 
%\be
%\label{eq:reg-loss}
%\sum_{(x,y) \in \S} \ell(\bftheta,x,y) + \frac{C}{p} \|\bftheta\|_p^p,
%\ee 
%defined over a  training set $\S$. The function $\ell$ measures the loss incurred in using $\bftheta$ to predict the label of $x$, given that the true label is $y$.

%In this paper we focus on structured SVMs and CRFs which are the most commonly used  models for structured prediction. The first definition of structured SVMs was given by  \cite{Taskar04} using the structured hinge loss
%$$\ell_{hinge}(\bftheta,x,y) = \max_{\hat y \in \Y} \left\{ e(y,\hat y) +  \bftheta^\top \Phi(x,\hat y) - \bftheta^\top \Phi(x,y)\right\}$$        
%where $e(y,\hat y)$ is some non-negative measure of error when predicting $\hat{y}$ instead of $y$ as the label of $x$. We assume that $e(y,y) = 0$, so that no loss is incurred for correct prediction. This loss function corresponds to a maximum-margin approach that explicitly penalizes training examples $(x,y)$ for which $\bftheta ^\top \Phi(x,y) < e(y,y_{\bftheta}(x)) + \bftheta ^\top \Phi(x,y_{\bftheta}(x))$.

%The second loss function that we consider is based on log-linear models, and is commonly used in CRFs, see \cite{Lafferty01}. Let the conditional distribution be $$p(\hat y|x,y;\bftheta) = \frac{1}{Z(x,y)} \exp\left(e_y(\hat y) + \bftheta^\top \Phi(x,\hat y)\right), \hspace{1cm} Z(x,y) = \sum_{\hat y} \exp\left(e_y(\hat y) + \bftheta^\top \Phi(x,\hat y) \right)$$
%where $e_y(\hat y) = e(y,\hat y)$ corresponds to a prior distribution, and $Z(x,y)$ is the partition function. The loss function is then the negative log-likelihood under the parameters $\bftheta$
%$$\ell_{log}(\bftheta,x,y) =  \ln \frac{1}{p(y|x,y;\bftheta)}.$$
%In both structured SVMs and CRFs a convex loss function and a convex regularization term are minimized. 


\section{Descent Algorithms for Structured Prediction}

Gradient-based methods are typically used to minimize the structured prediction objective. CRFs and structured SVMs however inherently differ in the properties of their loss functions. While CRFs have a smooth objective and gradient descent can be directly applied, structured SVMs  are described by the non-smooth hinge-loss, therefore  subgradient  methods are employed. 
In the following we describe a gradient descent algorithm for CRFs and a subgradient descent algorithm  for structured-SVMs due to \cite{Lebanon02,Ratliff06}. 

In CRFs one aims to minimize  the regularized negative log-likelihood  of the conditional distribution $p(\hat y|x,y;\bftheta)$ which decomposes  into the log-partition $Z(x,y)$ term and the linear term $\bftheta^\top \Phi(x,y)$. Hence the problem of minimizing the regularized loss  with the loss function  $\ell_{log}$ can be written as 
$$\mbox{(CRF)} \hspace{2cm} \min_{\bftheta} \left\{  \sum_{(x,y) \in \S} \ln Z(x,y) - \bfd^\top \bftheta + \frac{C}{p} \|\bftheta\|_p^p \right\},$$
where $(x,y)\in \S$ ranges over the training pairs and 
\begin{equation}
\bfd =  \sum_{(x,y) \in \S} \Phi(x,y)
\label{eq:em}
\end{equation}
is the vector of empirical means. In coordinate descent methods,  each coordinate $\theta_r$ is iteratively updated in the direction of the negative gradient, for some step size $\eta$. The gradient of the log-partition function corresponds to the probability distribution $p(\hat y | x,y ; \bftheta)$, and the direction of descent takes the form $$\sum_{(x,y) \in \S} \sum_{\hat y} p(\hat y | x,y ; \bftheta) \phi_r(x,\hat y) - d_r +|\theta_r|^{p-1} \mbox{sign}(\theta_r).$$

\vspace{0.5cm}
Structured SVMs aim at minimizing the regularized hinge loss $\ell_{hinge}(\bftheta,x,y)$, which measures the loss of the label $y_{\bftheta}(x)$ that most violates the training pair $(x,y) \in \S$ by more than $e(y,y_{\bftheta}(x))$. Since $y_{\bftheta}(x)$ is independent of the training label $y$, the structured SVM program takes the form: 
$$\mbox{(structured SVM)} \hspace{2cm} \min_{\bftheta}  \left\{ \sum_{(x,y) \in \S} \max_{\hat y \in \Y} \left\{e(y,\hat y) + \bftheta^\top \Phi(x,\hat y) \right\} -  \bfd^\top \bftheta  + \frac{C}{p}\|\bftheta\|_p^p \right\},$$
where $(x,y)\in \S$ ranges over the training pairs, and $\bfd$ is the vector of empirical means defined in (\ref{eq:em}). The structured SVM objective involves the max function, hence it is not smooth. However every convex function $f(\bftheta)$ has a {\em subdifferential}, denoted by $\partial f(\bftheta)$, which is the family of {\em subgradients}, i.e. supporting hyperplanes to its epigraph at $(\bftheta,f(\bftheta))$. The subdifferential generalizes the concept of the gradient since a convex function is smooth if and only if its subdifferential consists of a single vector, i.e. its gradient (cf. \cite{Bertesekas03} Theorem 4.2.2). Danskin's theorem (cf. \cite{Bertesekas03}, Theorem 4.5.1) states that the subdifferential of the max function corresponds to the probability distributions $p(y^* | x,y ; \bftheta)$ over the optimal set $\Y^* = \mbox{argmax}_{\hat y \in \Y} \left\{e(y,\hat y) + \bftheta^\top \Phi(x,\hat y) \right\}$, therefore the subdifferential of the structured SVM takes the form $$\sum_{(x,y) \in \S} \sum_{y^* \in \Y^*} p(y^* | x,y ; \bftheta) \phi_r(x,y^*) - d_r +|\theta_r|^{p-1} \cdot \mbox{sign}(\theta_r)$$
Unlike the smooth case, a negative subgradient not necessarily points towards a direction of descent, therefore subgradient methods are usually not monotonically decreasing, and depend on the step size. Their optimal solution is taken from the algorithm sequence.  

\vspace{0.5cm}
In the following we deal with both structured prediction tasks (i.e., structured SVMs and CRFs) as two instances of the same framework, extending the partition function to norms, namely $Z_\epsilon(x,y) = \|\exp \left(e_y(\hat y) + \bftheta^\top \Phi(x,\hat y) \right) \|_{1/\epsilon}$, where the norm is computed for the vector ranging over $\hat y \in \Y$. Using the norm formulation we move from the partition function, for $\epsilon=1$, to the maximum over the exponential function for $\epsilon=0$. Equivalently, we relate the log-partition and the max-function by the soft-max function 
\be
\label{eq:soft-max}
\ln Z_\epsilon(x,y) = \epsilon \ln \sum_{\hat y} \exp \left(  \frac{e_y(\hat y) + \bftheta^\top \Phi(x,\hat y)}{\epsilon} \right) 
\ee
For $\epsilon=1$ the soft-max function reduces to the log-partition function, and for $\epsilon=0$ it reduces to the max-function. Moreover, for $\epsilon \rightarrow 0$ the soft-max function is a smooth approximation of the max-function, in the same way the $L_{1/\epsilon}$-norm is a smooth approximation of the $L_\infty$-norm. This smooth approximation of the max-function is a common practice, cf. \cite{Vontobel06}, \cite{Johnson07}. We thus define the structured prediction problem as
\be
\label{eq:sp}
\mbox{(structured-prediction)} \hspace{2cm} \min_{\bftheta} \left\{  \sum_{(x,y) \in \S} \ln Z_\epsilon(x,y) - \bfd^\top \bftheta + \frac{C}{p} \|\bftheta\|_p^p \right\},
\ee
which is a one-parameter extension of CRFs and structured SVMs, for $\epsilon =1$ and $\epsilon=0$ respectively. Similarly to CRFs and structured SVMs, one can use gradient methods for structured prediction, whose gradient in the r-th coordinate $\theta_r$ takes the form
\be
\label{eq:grad}
\sum_{(x,y) \in \S} \sum_{\hat y} p_\epsilon(\hat y | x,y ; \bftheta) \phi_r(x,\hat y) - d_r +|\theta_r|^{p-1} \mbox{sign}(\theta_r),
\ee
where 
\be
\label{eq:pe}
p_\epsilon (\hat y | x,y ; \bftheta) = \frac{1}{Z_\epsilon(x,y)^{1/\epsilon}} \exp (e_y(\hat y) + \bftheta^\top \Phi(x,\hat y))^{1/\epsilon}
\ee 
is a probability distribution over the possible labels $\hat y \in \Y$. When $\epsilon \rightarrow 0$ this probability distribution gets concentrated around its maximal values, since all its elements are raised to the power of a very large number (i.e. $1/\epsilon$) normalized by $Z_\epsilon(x,y)$. Therefore for $\epsilon=0$ we get a subgradient of structured SVMs.

One can compute the soft-max (\ref{eq:soft-max}) and the probability $p_\epsilon (\hat y | x,y ; \bftheta) $ in (\ref{eq:pe}) using variational methods (cf. \cite{Wainwright08}, Theorem 8.1) since
\be
\label{eq:var}
\ln Z_\epsilon(x,y) = \max_{p(\hat y) \in \Delta_{\Y} }
\sum_{\hat y} p(\hat y) \left( e_y(\hat y) + \bftheta^\top \Phi(x,\hat y) \right) + \epsilon H(p),
\ee
where $\Delta_{\Y}$ is the set of all probability distribution over $\Y$, namely $p(\hat y) \ge 0$,  $\sum_{\hat y} p(\hat y)=1$, and $H(p)$ is the entropy of the probability distribution $p(\hat y)$. One can verify that the distribution $p_\epsilon(\hat y | x,y,\bftheta)$ in (\ref{eq:pe}) is the optimal argument of the program in (\ref{eq:var}), by differentiating and finding the vanishing point of the gradient. 


\section{Structured Prediction in Graphical Models}
In many real-life applications the labels $y \in \Y$ are $n$-tuples $y=(y_1,...,y_n)$, hence there are exponentially many labels in $\Y$. Due to memory and computational constraints it is not possible to use features $\phi_r(x,y)$ that have different values for every label $y \in \Y$. The feature maps usually describe relations between subsets of label elements $y_\alpha \subset \{y_1,...,y_n\}$, and local interactions on single label elements $y_v$, namely
\be
\label{eq:feature}
\phi_r(x,\hat y_1,...,\hat y_n) = \sum_{v \in V_{r,x}} \phi_{r,v}(x,\hat y_v) + \sum_{\alpha \in E_{r,x}} \phi_{r,\alpha}(x,\hat y_\alpha).
\ee
Each feature $\phi_r(x,\hat y)$ can be described by its {\em factor graph} $G_{r,x}$, which is a bipartite graph with one set of nodes corresponding to $V_{r,x}$ and the other set corresponds to $E_{r,x}$, \cite{Kschischang-Frey01}. An edge connects a single label node $v \in V_{r,x}$ with a subset of label nodes $\alpha \in E_{r,x}$ if and only if $y_v \in y_\alpha$. In the following we consider the factor graph $G = \cup_r G_r$ which is the union of all feature graphs. We denote by $N(v)$ and $N(\alpha)$ the set of neighbors of $v$ and $\alpha$ respectively, in the factor graph $G$. For notational simplicity we consider fully factorized priors
\be
\label{eq:prior}
e_y(\hat y_1,...,\hat y_n) = \sum_{v=1}^n e_{y,v}(\hat y_v),
\ee    
although our derivation naturally extends to any graphical model representing the local interactions of $e_y(\hat y)$. 

The local structure on the features (\ref{eq:feature}) in turn induces a local structure on the learning problem (\ref{eq:sp}). In particular, the gradient (\ref{eq:grad}) involves the average on the local features $\phi_{r,v}(x,\hat y_v), \phi_{r,\alpha}(x,\hat y_\alpha)$, therefore it considers the marginal probabilities $p_\epsilon(\hat y_v | x,y,\bftheta)$ and $p_\epsilon(\hat y_\alpha | x,y,\bftheta)$. Moreover, when the factor graph has no cycles, the probability distribution can be represented by a multiplication of its marginal probabilities, namely $p_\epsilon(\hat y | x,y,\bftheta) = \prod_\alpha p_\epsilon(\hat y_\alpha | x,y,\bftheta) \prod_v p_\epsilon(\hat y_v | x,y,\bftheta)^{1-|N(v)|}$. In this case, using the variational method (\ref{eq:var}), the soft-max function (\ref{eq:soft-max}) in the structured prediction objective can be efficiently computed given the marginal probabilities, where we replace the entropy function by local entropies over the marginal probabilities $\sum_\alpha H(p_\epsilon(\hat y_\alpha | x,y,\bftheta)) - \sum_v(1-{\scriptsize |N(v)|}) H(p_\epsilon(\hat y_v | x,y,\bftheta))$, \cite{yedidia05}.  

In general, when the graphical model has cycles, the structured prediction objective is exponentially hard to compute since the soft-max, $\ln Z_\epsilon(x,y)$,  considers exponentially many elements $\hat y \in \Y$. Similarly, the gradient requires the marginal probabilities, $p_\epsilon(\hat y_v | x,y ; \bftheta)$ and $p_\epsilon(\hat y_\alpha | x,y ; \bftheta)$, which involve summing over exponentially many elements. In the following we describe the approximate inference framework which is typically used to approximate the soft-max and the marginal probabilities. The approximate inference framework is based on the variational method in (\ref{eq:var}) which derives the soft-max by the marginal probabilities when the factor graph has no cycles. The main idea is to replace the marginal probabilities $p(\hat y_v | x,y,\bftheta), p(\hat y_\alpha | x,y,\bftheta)$ with beliefs $b_v(\hat y_v), b_\alpha(\hat y_\alpha)$ and the entropy term by local entropies. The approximation of (\ref{eq:var}) takes the form:
\begin{eqnarray}
\ln Z_\epsilon(x,y) &\approx& \max \sum_{v,\hat y_v} b_v(\hat y_v) \phi_v(x,\hat y_v) + \sum_{\alpha,\hat y_\alpha} b_\alpha(\hat y_\alpha) \phi_\alpha(x,\hat y_\alpha) + \epsilon \left( \sum_\alpha c_\alpha H(b_\alpha) + \sum_v c_v H(b_v) \right),  \nonumber \\
&& \mbox{subject to } \;\;\; b_v(\hat y_v) \in \Delta_{\Y_v}, \;\;\; b_\alpha(\hat y_\alpha) \in \Delta_{\Y_\alpha}, \;\;\; \sum_{\hat y_\alpha \setminus \hat y_v} b_\alpha(\hat y_\alpha) = b_v(\hat y_v), 
\label{eq:approx}
\end{eqnarray}
where $\Delta_{\Y_v}$ is the set of probability distributions over $\Y_v$, i.e. $b_v(\hat y_v) \ge 0$, $\sum_{\hat y_v} b_v(\hat y_v)=1$, and $\Delta_{\Y_\alpha}$ is the set of probability distributions over $\Y_\alpha$. Also, we used a short notation for the $\bftheta$ weighted features in the graphical model $\phi_v (x,\hat y_v) = e_y(\hat y_v) +  \sum_{r: v \in V_{r,x}} \theta_r \phi_{r,v}(x,\hat y_v)$ and $\phi_\alpha(x,\hat y_\alpha) = \sum_{r: \alpha \in E_{r,x}} \theta_r \phi_{r,\alpha}(x,\hat y_\alpha)$. 

The entropy approximation in (\ref{eq:approx}) is known as the fractional entropy approximation \cite{Wiegerinck03}. When the graphical model has no cycles, and the fractional entropy weights are chosen according to the Bethe entropy, i.e. $c_\alpha=1, c_v = 1-|N(v)|$, the variational program in (\ref{eq:approx}) is equivalent to the one in (\ref{eq:var}), and gives an exact characterization of the soft-max, and the beliefs are the true marginal probabilities. However, when the graphical model has cycles this variational program is an approximation of the soft-max and the marginal probabilities; no guarantees on the quality of the approximation are known so far. 

A common method for solving the approximate inference program in (\ref{eq:approx}) is to send messages along the edges of the factor graph. In the following we present a message-passing algorithm for solving the approximate inference problem, (cf. \cite{Pearl-88,Wainwright-05map,Wainwright-05upper,heskes06,Meltzer-uai09,Hazan09}). To follow the product form of beliefs propagation algorithm (BP) we set $\bar \phi_v(\hat y_v) = \exp(\phi_v(\hat y_v))$, and $\phi_\alpha(\hat y_\alpha) = \exp(\phi_\alpha(\hat y_\alpha))$. In this case the messages can be computed as
$$
m_{\alpha \rightarrow v}(\hat y_v)= \left\| \bar \phi_\alpha(\hat y_\alpha) \prod_{u \in N(\alpha)\setminus v}n_{u \rightarrow \alpha}(\hat y_u) \right\|_{1/\epsilon c_\alpha}, \hspace{1cm}
n_{v \rightarrow \alpha}(\hat y_v)\propto \frac{\left(\bar \phi_v(\hat y_v) \displaystyle \prod_{\beta \in N(v) \setminus \alpha}m_{\beta \rightarrow v}(\hat y_v) \right)^{c_\alpha / \hat c_v}}{m_{\alpha \rightarrow v}(\hat y_v)},$$
where the norm is computed for the vector ranging over $\hat y_\alpha$ while holding $\hat y_v$ fixed, and $\hat c_v = c_v+\sum_{\alpha \in N(i)} c_\alpha$ and $\propto$ indicates that the vector can be normalized. After convergence, one can infer the beliefs by
$$b_v(\hat y_v) \propto \left( \bar \phi_v(\hat y_v) \prod_{\alpha \in N(v)} m_{\alpha \rightarrow v}(\hat y_v) \right)^{1/\epsilon c_v}, \hspace{1cm} b_\alpha(\hat y_\alpha) \propto  \left( \bar \phi_\alpha(\hat y_\alpha)\prod_{u \in N(\alpha)} n_{u\rightarrow \alpha}(\hat y_u) \right)^{1/\epsilon c_\alpha},$$

When the factor graph has no cycles, one can use the above message-passing algorithm with the Bethe entropy, i.e. $c_\alpha=1$ and $c_v=1-|N(v)|$ to compute in linear time the soft-max, $\ln Z_\epsilon(x,y)$, and the marginal probabilities, $p_\epsilon(\hat y_v | x,y ; \bftheta)$ and $p_\epsilon(\hat y_\alpha | x,y ; \bftheta)$, therefore it can be used as a subroutine to compute the structure prediction objective and gradient. Focusing on the Bethe entropy, this message-passing algorithm is the $\epsilon$ parameter extension of the BP algorithm, which includes as special cases the sum-product for $\epsilon=1$ and the max-product for $\epsilon=0$. It  can be shown that for every positive $\epsilon$ this BP extension solves exactly (\ref{eq:var}) for graphs without cycles, since by using a change of variables it reduces to the sum-product algorithm for $\epsilon > 0$.
 
When the factor graph has cycles this message-passing algorithm has in general no guarantees for convergence (unless $c_\alpha,c_v >0$), nor on the number of iterations, nor on the quality of the solution, and it is used as an {\em approximation} for the soft-max and the marginal probabilities. Therefore one encounters  two important problems when dealing in structured prediction with  graphs with cycles:  The first one is its efficiency, as for graphs with cycles there are no guarantees on the number of steps the message-passing algorithm requires till convergence, therefore it is computationally costly to run it as subroutine for more that few hundred iterations. The second problem is accuracy, as the message-passing algorithm has no guarantees on the quality of the solution, therefore the gradient and the objective function can only be approximated, and one cannot know if the update rule decreases or increases the structured prediction objective. 

In contrast, in this work  we propose to approximate the structured prediction problem and to efficiently solve the approximated problem exactly by message-passing.  This allows us to efficiently learn large scale graphical models. 

